Interpreting convolutional neural networks' low dimensional approximation to quantum spin systems

Convolutional neural networks (CNNs) have been employed along with Variational Monte Carlo methods for finding the ground state of quantum many-body spin systems with great success. In order to do so, however, a CNN with only linearly many variational parameters has to circumvent the ``curse of dimensionality'' and successfully approximate a wavefunction on an exponentially large Hilbert space. In our work, we provide a theoretical and experimental analysis of how the CNN optimizes learning for spin systems, and investigate the CNN's low dimensional approximation. We first quantify the role played by physical symmetries of the underlying spin system during training. We incorporate our insights into a new training algorithm and demonstrate its improved efficiency, accuracy and robustness. We then further investigate the CNN's ability to approximate wavefunctions by looking at the entanglement spectrum captured by the size of the convolutional filter. Our insights reveal the CNN to be an ansatz fundamentally centered around the occurrence statistics of $K$-motifs of the input strings. We use this motivation to provide the shallow CNN ansatz with a unifying theoretical interpretation in terms of other well-known statistical and physical ansatzes such as the maximum entropy (MaxEnt) and entangled plaquette correlator product states (EP-CPS). Using regression analysis, we find further relationships between the CNN's approximations of the different motifs' expectation values. Our results allow us to gain a comprehensive, improved understanding of how CNNs successfully approximate quantum spin Hamiltonians and to use that understanding to improve CNN performance.

==> NewTexFiles0415/Motif_MaxEnt.tex <==
\begin{comment}
    We can also formulate a MaxEnt ansatz over the motif equivalence classes $\{M_n\}$ by picking a representative string $s'_n$ for each motif equivalence class $\{M_n\}$:
\begin{equation}
       \ln \psi^{\mathrm{MaxEnt}}(s)=\sum_n \lambda_n m_{s'_n}(s) +\ln Z
\end{equation}
\end{comment}

\section{Note on operators and Lagrange multipliers}
\label{suppl:Lagrange_mult}
The MaxEnt formalism only requires two ingredients: an orthonormal basis and a set of independent operators. If the operators are all diagonal, we can make a `moment matrix' in which the rows and columns correspond to the operators and basis elements, as shown in Fig.~\ref{fig:CNN-arch}. The rank of this matrix determines the number of independent operators. If the rank is equal to the number of operators, then we can proceed with the derivation from the MaxEnt section. However, if the rank is less than the number of operators, then that means there is some redundancy in the operators, which would correspond to redundancy in the Lagrange multipliers, i.~e.~if $q$ is the number of operators and $p$ is the rank of the operator matrix and $q-p=j$, then every set of Lagrange multipliers belongs to a $j$-dimensional degenerate manifold. There are two issues that arise when $j>0$:
\begin{enumerate}
    \item There is no meaningful way to compare two different values of the Lagrange multipliers since a single Lagrange multiplier can belong to many different manifolds, and conversely, a single wavefunction can have many different values of the Lagrange multipliers
    \item The MaxEnt formalism requires solving a system of equations to obtain the unique MaxEnt wavefunction. If there are more equations than independent variables, an algebraic solution will likely fail due to numerical instability, despite the fact that a solution should exist (e.~g.~solving the system of equations $\{x=2,x=2+10^{-10}\}$ will fail if it looks for an exact solution)
\end{enumerate}
To get rid of both of these issues, the natural way is to simply choose $p$ operators instead of $q$ operators (while preserving the rank of the operator matrix). This can always be done in practice by row reducing the operator matrix. Let $o_1,\ldots,o_p$ be a choice of independent operators (not necessarily unique), and $o_{p+1},\ldots,o_q$ be the redundant operators, which can all be written as linear combinations of the independent operators $o_k=\sum_{i=1}^pc_{ik}o_i$. Then the MaxEnt wavefunction looks like
\begin{align}
    \ln\psi^{(MaxEnt)}(s)&=\sum_{i=1}^q\lambda_io_i(s)\\
    &=\sum_{i=1}^p\lambda_io_i(s)+\sum_{k=p+1}^q\lambda_ko_k(s)\\
    &=\sum_{i=1}^p\lambda_io_i(s)+\sum_{k=p+1}^q\lambda_k\sum_{i=1}^pc_{ik}o_i(s)\\
    &=\sum_{i=1}^p\lambda_io_i(s)+\sum_{i=1}^po_i(s)\sum_{k=p+1}^q\lambda_kc_{ik}\\
    &=\sum_{i=1}^p\left(\lambda_i+\sum_{k=p+1}^q\lambda_kc_{ik}\right)o_i(s)\\
    &=\sum_{i=1}^p\lambda_i^*o_i(s)
\end{align}
As expected, a redundant MaxEnt wavefunction can always be expressed as a non-redundant MaxEnt wavefunction. If we fix $\lambda_k$ for all $k>p$, then $\lambda_i$ and $\lambda_i^*$ are simply related by a constant shift, so they are essentially interchangeable. However, if the $\lambda_k$s are varied alongside the $\lambda_i$s, then this might no longer be true.

Now we can examine the case of a 1D M=2 spin chain with motif count operators. The number of operators is $2^K$, and the rank of the motif count matrix is $2^{K-1}$ for $N>2K$ (found empirically). Therefore there is a set of $2^{K-1}$ independent operators. Empirically, we find that any set of $2^{K-1}$ operators is independent if it does not contain two conjugate operators ($m_{s'}$ and $m_{\Bar{s'}}$). For the CNN, the objects which act like Lagrange multipliers are the motif activations $v(s')$ times the output weight $w_0$. If the grand sum condition holds, then the preactivations of $s'$ and $\Bar{s'}$ will have opposite sign, which guarantees that one of the two activations is 0. Therefore, we can choose an independent set of operators to be all the operators whose substring activations are nonzero. The rest of the Lagrange multipliers are all 0. Hence there was never actually any redundancy in the CNN to begin with (if the grand sum condition holds). If we instead used a CNN without the ReLU activation, then $\lambda_i^*$ are no longer free parameters.

As a concrete example, we can examine the case of $M=K=2$. The four redundant operators are $\{m_{\uparrow\uparrow},m_{\uparrow\downarrow},m_{\downarrow\uparrow},m_{\downarrow\downarrow}\}$, and they satisfy the equations $\{m_{\uparrow\uparrow}=m_{\downarrow\downarrow},m_{\uparrow\downarrow}=m_{\downarrow\uparrow}\}$. Choosing $\{m_{\uparrow\uparrow},m_{\uparrow\downarrow}\}$ as the set of independent operators, we end up with $\{\lambda_{\uparrow\uparrow}^*=\lambda_{\uparrow\uparrow}+\lambda_{\downarrow\downarrow},\lambda_{\uparrow\downarrow}^*=\lambda_{\uparrow\downarrow}+\lambda_{\downarrow\uparrow}\}$. In order to have a well-behaved model, $\lambda_{\uparrow\uparrow}^*$ and $\lambda_{\uparrow\downarrow}^*$ need to be free parameters, which is why the CNN needs the ReLU activation. Otherwise (assuming the grand sum condition) we would have $\lambda_{\uparrow\uparrow}^*=\lambda_{\uparrow\downarrow}^*=0$. Of course, in the CNN the $\lambda_{s'}^*$ are not truly free parameters because they are functions of the CNN parameters, but those constraints depend on the model, rather than the intrinsic structure of the operators.


==> NewTexFiles0415/RelatedWork.tex <==
\subsection*{Related Work}

==> NewTexFiles0415/scratch.tex <==

% \subsection{Group theory interpretation: Equivalence to Convolution}
% The expression in Eq.~\eqref{eq:CNN_arch} can be rewritten in terms of convolution w.r.t. the cyclic group:
% \begin{eqnarray}
% \frac{\ln \psi(s)}{v} &=&
% \sum_{i=1}^N \sigma \Big(\langle w, s_{i:i+K-1} \rangle + b \Big) \nonumber \\
% &=& \sum_{i=1}^{N}\sigma(\langle T^{i}w, s \rangle+b) \nonumber \\ 
% &=& j^{T}\sigma(w * s+b), \label{eq:group_trans}
% \end{eqnarray}
% where we slightly abuse $w$ to denote a kernel of size $M \times N$ instead of $M \times K$, starting from the second line in Eq.~\eqref{eq:group_trans} and $supp(w)=[1,\cdots,K]$. $T$ is the generator of cyclic shifts of the group $\mathcal{C}$, the cyclic group, and $j$ is the all-ones vector. We define $\sigma:\mathbb{R} \to \mathbb{R}$ as the non-linearity function. In the third line of Eq.~\eqref{eq:group_trans} we also slightly abuse it as function from $\mathbb{R}^{M \times N}$ to $\mathbb{R}^{M \times N}$, with element-wise nonlinearity.

% \begin{wraptable}{r}{8cm}
%     \begin{center}
%         \caption{Regression Results for $\delta_r(E_0)$ vs. $e^{-\bar{\delta}_d}$, $d \in \{0, 1, 2\}$. $R^2 = .923$, \# Obs. $= 160$, Cond. No. $= 131$.}
%         \label{tab:reg_error_moment}
%         % [20220503] Refered to: https://www.csus.edu/indiv/v/vangaasbeckk/courses/145/sup/regressionresults.pdf
%         \begin{tabular}{rr}
%             \toprule
%             Variable & Coeffcient (std.) \\
%             \midrule
%             Intercept & $-.449\text{**}(.072)$ \\
%             $e^{-\bar{\delta}_0}$ & $.149\text{**}(.016)$ \\
%             $e^{-\bar{\delta}_1}$ & $.363\text{**}(.061)$ \\
%             $e^{-\bar{\delta}_2}$ & $.251\text{**}(.059)$ \\
%             $K$ $(10^{-2})$ & $-2.84\text{**}(0.56)$  \\
%             \texttt{init} $(10^{-2})$ & $-7.06\text{*}(2.11)$ \\
%             \texttt{force} $(10^{-2})$ & $-4.98^\dagger(2.11)$ \\
%             \texttt{CPS} & $-.106\text{**}(.023)$ \\
%             $\log n_{\mathrm{opt}}$ $(10^{-3})$ & $-9.06(6.64)$ \\
%             $\log \eta$ $(10^{-4})$ & $1.40(6.57)$ \\
%             \bottomrule
%         \end{tabular}
%     \end{center}
%     Units of the coefficients are labeled in parentheses after the variable names. $\dagger$, *, ** indicate significance at the 95\%, 99\% and 99.9\% level, respectively.
% \end{wraptable}

% \subsection{Tuning learning rates and \texttt{n\_opt} in Large N cases} \label{suppsec:tuning_results}
% Since we have seen the impact of \texttt{n\_opt} on the final model performance in a smaller spin chain, we also perform similar experiments on larger cases where $N = 30$ or $60$. See Fig. \ref{fig:E_tuning}. We find that when all else equal:
% \begin{enumerate}
%     \item Larger \texttt{n\_opt} improves prediction when the learning rate is not too large.
%     \item Models trained with larger \texttt{lr} generally have a better performance after training a fixed number of iterations (500) when the learning rate is not too large.
%     \item When \texttt{lr} and \texttt{n\_opt} are both large, the performance may even get worse while taking a lot of time on the sample reuse iterations.
%     \item There is not much difference between using kernel size $K = 6$, $12$ and $24$ but $K = 3$ is definitely not sufficient.
%     \item Our proposed algorithm performs better than the original one even we tune the learning rate and \texttt{n\_opt}, which corresponds to the best run in each row for each algorithm.
% \end{enumerate}

% In Fig. \ref{fig:a_tuning}, we show the number of iterations required to achieve a prediction error of less than 0.1 for different configurations. If the algorithm never achieves a small error, we set this iteration number to the total number of training iterations, which is 500 in this case. Note that serves as a lower bound, meaning if we were to train the models for more iterations, the number of required iterations for bad configurations could be longer. We observe that when all else equal:
% \begin{enumerate}
%     \item Larger \texttt{n\_opt} reduces the required number of iterations when \texttt{lr} is not too large, since sampling reuse effectively adds iterations to the inner loop, while we count the iteration of the outer loop only.
%     \item Larger \texttt{lr} also reduces the required number of iterations when \texttt{n\_opt} is not too large, since all \texttt{lr} values we tested are in a reasonable range.
%     \item When \texttt{lr} and \texttt{n\_opt} are both large, the performance may even get worse while taking a lot of time on the sample reuse iterations.
%     \item There is not much difference no matter what $K$ we use for our proposed algorithms. However, the original algorithm needs a larger kernel size to be able to achieve a decent accuracy fast enough.
%     \item The original algorithm is very sensitive to initial conditions, especially for a larger $N$.
%     \item Our proposed algorithms required much fewer iterations to achieve a good enough accuracy.
% \end{enumerate} 

% \begin{figure}[!h]
%      \centering
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/energy_N30_tuning.png}
%          \caption{$N = 30$}
%          \label{fig:E_N30_tuning}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/energy_N60_tuning.png}
%          \caption{$N = 60$}
%          \label{fig:E_N60_tuning}
%      \end{subfigure}
%         \caption{Predicted energy vs \# of sample reuse iterations. Each row shows a different kernel size, while each column shows a different learning rate. Each setting contains 5 random seeds. We can see that our proposed algorithm performs better than the original one even we tune the learning rate and \texttt{n\_opt}, which corresponds to the best run in each row for each algorithm.}
%         \label{fig:E_tuning}
% \end{figure}

% \begin{figure}[!h]
%      \centering
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/achieving_acc_N30_tuning.png}
%          \caption{$N = 30$}
%          \label{fig:a_N30_tuning}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/achieving_acc_N60_tuning.png}
%          \caption{$N = 60$}
%          \label{fig:a_N60_tuning}
%      \end{subfigure}
%         \caption{Number of iterations required to achieve a prediction error less than 0.1 vs \# of sample reuse iterations. Each row shows a different kernel size, while each column shows a different learning rate. Each setting contains 5 random seeds. We can see that our proposed algorithm performs better than the original one under all circumstances.}
%         \label{fig:a_tuning}
% \end{figure}

% \subsection{Impact of Initialization} \label{suppsec:impact_of_init}
% In our analysis of the experiments, we find that the number of positive motif activations at initialization, denoted by $N_a^+$, correlates with the quality of CNN predictions. For example, in Fig. \ref{fig:Na_plus_N8}, we show the box plots of final fidelity vs \# of positive motif activations at initialization, where N = 8. Each row shows a different learning rate and each column shows a different algorithm. The horizontal axis shows $N_a^+$ and the vertical axis shows the final fidelity. The red dotted line shows the fidelity of predictions given by a model in the failure mode (see in Appendix Section \ref{ap:sec:failure}). For each combination of a row, column, and color, 10 random seeds are used. We can observe that in the original algorithm when $N_a^+$ is either too small or too large, the model will converge to one of the failure modes mentioned in Appendix Section \ref{ap:sec:failure}. On the contrary, our grand sum initialization controls $N_a^+$ well in the sweet spot, which is exactly $2^{K-1}$. In addition, we can see that when all else is equal, a larger number of sample reuse iteration (\texttt{n\_opt}) improves final fidelity, and models trained with larger learning rates converge faster. However, when the learning rate and \texttt{n\_opt} are both large, some models will not get improved, and they will even fail to converge to fidelity 1. Hence, using a large learning rate and an intermediate number of sample reuse can result in a good model with low time costs.

% \begin{figure}[!h]
%      \centering
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/Na_plus_N8_K4.png}
%          \caption{$K = 4$}
%          \label{fig:Na_plus_N8_K4}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/Na_plus_N8_K5.png}
%          \caption{$K = 5$}
%          \label{fig:Na_plus_N8_K5}
%      \end{subfigure}
%         \caption{Box plots of final fidelity vs \# of positive motif activations at initialization, where $N = 8$. Each row shows a different learning rate and each column shows a different algorithm. The horizontal axis shows $N_a^+$ and the vertical axis shows the final fidelity. The red dotted line shows the fidelity of predictions given by a model in the failure mode. For each combination of a row, column, and color, 10 random seeds are used. This shows that using a large learning rate and an intermediate number of sample reuse can result in a good model with low running time.}
%         \label{fig:Na_plus_N8}
% \end{figure}

% \section{Regression Analysis}


% Here we describe the details of how we train the CPS ansatz and collect data for the regression analysis.
% \subsection{Data Collection} \label{suppsubsec:regression_data}
% We adapt the variational CNN training scheme for CPS models parameterized using Eq.~\eqref{eq:unify} and set $\mathcal{C}_{s'}$, $\forall s^\prime \in \mathcal{M}_{M, K}$ as our trainable parameters.

% We focus on the $N=60$ system and examine the models with $L = F = 1$ and $K \in \{3, 6\}$. There are 20 groups of motifs in total according to the MEV distance. The learning rates $\eta \in \{0.0001, 0.001\}$, the numbers of sample reuse during optimization $n_{\mathrm{opt}} \in \{10, 100\}$, and  the training algorithms $\mathcal{A} \in$ \{\texttt{original}, \texttt{grand} \texttt{-} \texttt{sum} \texttt{-} \texttt{init}, \texttt{grand} \texttt{-} \texttt{sum} \texttt{-force}, \texttt{CPS}$\}$. Each setting is run 5 times with different random intialization.




% We group degenerate motifs into their own `equivalence classes', such that two motifs are in the same equivalence classes if their ground state MEVs are identical. We order the motif equivalence classes in terms of descending MEV values, resulting in the Neel motifs being the first one, with the MEV distance $d$ being how far an motif equivalence class is from the Neel motif class (the Neel motif class has $d=0$).

% \subsection{Regression Results} \label{suppsec:E_relerr_regression_results}


% \textcolor{red}{I think this paragraph can be moved to Supplement for Science: it's fine to have it here for arxiv}
% In Table \ref{tab:reg_error_moment}, we show our best regression, model (ii) (see Sec. \ref{suppsubsec:regression} for results of model (i) and (iii)). The boolean variables \texttt{init}, \texttt{force} and \texttt{CPS} indicate whether the corresponding algorithms are used. All coefficients for the MEV errors are statistically significant. The signs indicate that overestimating $\bar{\delta}_d$ leads to less $\delta_E$, consistent with our analysis based on Fig. \ref{fig:drE_vs_drmu}. Some hyperparameters also have statistical significance, even though they do not have direct impact on $\delta_E$. Since we only focus on 3 out of 20 groups of motifs, the coefficients for the hyperparameters must capture the variation in groups of motifs unselected for regression. Thus, by using \texttt{grand} \texttt{-} \texttt{sum} \texttt{-} \texttt{init}, \texttt{grand} \texttt{-} \texttt{sum} \texttt{-force} or \texttt{CPS}, which have negative coefficients, we are able to reduce $\delta_E$ by assigning more proper MEVs to the motifs. Note that \texttt{CPS} has the largest absolute value, indicating CPS models provide a more accurate approximation of the ground state energy.

% \subsection{Additional Regression Results} \label{suppsubsec:regression}
% Model (i) uses linear features and (iii) use the motifs with the least MEVs. See Table \ref{tab:reg_error_moment_i} for the regression results for model (i) and Table \ref{tab:reg_error_moment_iii} for model (iii). We can interpret the coefficient in Table \ref{tab:reg_error_moment_i} similarly to model (ii) in Sec. \ref{suppsec:E_relerr_regression_results}. However, for model (iii), we can see that the coefficients of $\bar{\delta}_d$, $d \in \{17, 18, 19\}$ have a much lower magnitude than those of $\bar{\delta}_d$, $d \in \{0, 1, 2\}$ in model (i) and (ii), indicating the least important MEVs do not contribute much to the prediction of the ground state energy.
% \begin{table}[h]
%     \begin{center}
%         \caption{Regression Results for $\delta_E$ vs. $\bar{\delta}_d$, $d \in \{0, 1, 2\}$. $R^2 = .865$, \# Obs. $= 160$, Cond. No. $= 132$.}
%         \label{tab:reg_error_moment_i}
%         % [20220503] Refered to: https://www.csus.edu/indiv/v/vangaasbeckk/courses/145/sup/regressionresults.pdf
%         \begin{tabular}{ccccc}
%             \toprule
%             Intercept & $\bar{\delta}_0$ $(10^{-2})$ & $\bar{\delta}_1$ & $\bar{\delta}_2$ & $K$ $(10^{-2})$ \\
%             \midrule
%             $.455\text{**}(.082)$ & $-8.25\text{**}(2.06)$ & $-.404\text{**}(.093)$ & $-.543\text{**}(.083)$ & $-3.95\text{**}(0.74)$ \\
%             \bottomrule
%         \end{tabular} \\
%         \begin{tabular}{ccccc}
%             \toprule
%             \texttt{init} $(10^{-2})$& \texttt{force} $(10^{-2})$& \texttt{CPS} & $\log n_{\mathrm{opt}}$ $(10^{-2})$ & $\log \eta$ $(10^{-3})$ \\
%             \midrule
%             $-8.81\text{*}(2.77)$ & $-5.00^\dagger(2.79)$ & $-.136\text{**}(.029)$ & $-1.18(.89)$ & $1.03(8.86)$ \\
%             \bottomrule
%         \end{tabular} \\
%     \end{center}
%     Units of the coefficients are labeled in parentheses after the variable names. Standard errors are reported in parentheses after the coefficients. $\dagger$ indicates significance at the 90\% level. * indicates significance at the 99\% level. ** indicates significance at the 99.9\% level.
% \end{table}

% \begin{table}[h]
%     \begin{center}
%         \caption{Regression Results for $\delta_E$ vs. $\bar{\delta}_d$, $d \in \{17, 18, 19\}$. $R^2 = .622$, \# Obs. $= 160$, Cond. No. $= 6.15\times 10^5$.}
%         \label{tab:reg_error_moment_iii}
%         % [20220503] Refered to: https://www.csus.edu/indiv/v/vangaasbeckk/courses/145/sup/regressionresults.pdf
%         \begin{tabular}{ccccc}
%             \toprule
%             Intercept & $\bar{\delta}_{17}$ $(10^{-3})$ & $\bar{\delta}_{18}$ $(10^{-4})$ & $\bar{\delta}_{19}$ $(10^{-6})$ & $K$ $(10^{-4})$ \\
%             \midrule
%             $.366\text{*}(.140)$ & $-1.97^\dagger(0.93)$ & $-5.02\text{**}(.98)$ & $-3.30^\dagger(1.33)$ & $-4.28(114.56)$ \\
%             \bottomrule
%         \end{tabular} \\
%         \begin{tabular}{ccccc}
%             \toprule
%              \texttt{init} $(10^{-2})$& \texttt{force} $(10^{-2})$ & \texttt{CPS} & $\log n_{\mathrm{opt}}$ $(10^{-2})$ & $\log \eta$ $(10^{-2})$ \\
%             \midrule
%             $-2.60(0.49)$ & $-2.33(0.49)$ & $-.129^\dagger(.050)$ & $2.34(1.44)$ & $3.12(1.43)$ \\
%             \bottomrule
%         \end{tabular} \\
%     \end{center}
%     Units of the coefficients are labeled in parentheses after the variable names. Standard errors are reported in parentheses after the coefficients. $\dagger$ indicates significance at the 95\% level. * indicates significance at the 99\% level. ** indicates significance at the 99.9\% level.
% \end{table}

% \subsection{Imposing Reflection Symmetry into CNN} \label{supp:bake}
% Original CNN:
% \begin{align}
%     \ln \psi(s) =& \sum_{f=1}^F v_f \sum_{i \in [N]} \sigma \Big(\langle T^i w_f, s \rangle + b_f \Big), \label{eq:ori_1}
% \end{align}
% Incorporate reflection symmetry at the \textbf{input} level:
% \begin{align}
%     \ln \psi^\dagger(s) =& 
%     \ln \psi(s + Rs) \nonumber \\
%     =& \sum_{f=1}^F v_f \sum_{i \in [N]} \sigma \Big(\langle T^i \tilde{w}_f, s + Rs\rangle \Big), \label{eq:rev_1}
% \end{align}
% Incorporate reflection symmetry at the \textbf{output} level:
% \begin{align}
%     \ln \psi^\ddagger(s) =& 
%     \ln \psi(s) + \ln \psi(Rs) \nonumber \\
%     =& \sum_{f=1}^F v_f \sum_{i \in [N]} \Big[ \sigma \big(\langle T^i \tilde{w}_f, s\rangle \big) + \sigma \big(\langle T^i \tilde{w}_f, Rs\rangle \big)\Big], \label{eq:rev_2}
% \end{align}


% When $F = 1$ and the GrandSum condition holds, we have
% \begin{align}
%     \frac{\ln \psi^\dagger(s)}{v}
%     =& \sum_{i=1}^N \sigma \Big(\langle T^i \tilde{w}, s + Rs\rangle \Big) \nonumber \\
%     =& \sum_{i=1}^N \sigma \bigg( \sum_{j=1}^N \langle \tilde{w}_{j-i}, s_j + (Rs)_j \rangle \bigg) \nonumber \\
%     =& \sum_{i=1}^N \bigg( \sum_{j=1}^N \langle \tilde{w}_{j-i}, s_j + (Rs)_j \rangle - \beta_i^\dagger \langle T^i \tilde{w}, s + Rs \rangle \bigg) \nonumber \\
%     =& \sum_{j=1}^N \bigg \langle \sum_{i=1}^N \tilde{w}_{j-i}, s_j + (Rs)_j \bigg \rangle - \sum_{i=1}^N \beta_i^\dagger \langle T^i \tilde{w}, s + Rs \rangle \nonumber \\
%     =& N \mathrm{grandsum}(\tilde{w}) - \sum_{i=1}^N \beta_i^\dagger \langle T^i \tilde{w}, s + Rs \rangle, \label{eq:rev_in_s}
% \end{align}
% where $\beta_i^\dagger = 1$, if $\langle T^i \tilde{w}, s + (Rs) \rangle < 0$; otherwise $\beta_i^\dagger = 0$.

% For the label-switched string, we have
% \begin{align}
%     \frac{\ln \psi^\dagger(Ls)}{v}
%     =& N \mathrm{grandsum}(\tilde{w}) - \sum_{i=1}^N \beta_i^{\dagger\prime \prime} \langle T^i \tilde{w}, Ls + RLs \rangle, \label{eq:rev_in_Ls}
% \end{align}
% where $\beta_i^{\dagger\prime\prime} = 1$, if $\langle T^i \tilde{w}, Ls + RLs \rangle < 0$; otherwise $\beta_i^{\dagger\prime\prime} = 0$.

% Note that $\langle T^i \tilde{w}, s + Rs \rangle + \langle T^i \tilde{w}, Ls + RLs \rangle = 2\mathrm{grandsum}(\tilde{w})$. Then, Taking Eq. (\ref{eq:rev_in_Ls}) - (\ref{eq:rev_in_s}), we have
% \begin{align}
%     \frac{\ln \psi^\dagger(Ls) - \ln \psi^\dagger(s)}{v}
%     =&  - \sum_{i=1}^N \beta_i^{\dagger\prime \prime} \langle T^i \tilde{w}, Ls + RLs \rangle \nonumber \\
%     &+ \sum_{i=1}^N \beta_i^\dagger \langle T^i \tilde{w}, s + Rs \rangle \nonumber \\ 
%     =& \sum_{i=1}^N (1 - \beta_{i}^\dagger) \langle T^{i} \tilde{w}, s + Rs \rangle \nonumber \\ 
%     &+ \sum_{i=1}^N \beta_i^\dagger \langle T^i \tilde{w}, s + Rs \rangle \nonumber \\
%     =& \sum_{i \in \{k | \beta_k^\dagger = 0\}} \langle T^i \tilde{w}, s + Rs \rangle \nonumber \\
%     &+ \sum_{i \in \{k | \beta_k^\dagger = 1\}} \langle T^i \tilde{w}, s + Rs \rangle \nonumber \\
%     =& \sum_{i=1}^N \langle T^i \tilde{w}, s + Rs \rangle \nonumber \\
%     =& N \mathrm{grandsum}(\tilde{w}).
% \end{align}
